Action-Value Calibration via Continuation Sharing for Long-Horizon Agentic Reinforcement Learning

Reinforcement learning for long-horizon agents relies on feedback from sequences of interactions, making credit assignment to individual actions difficult. Existing methods such as GiGPO compare actions at shared states to compute relative advantages, but estimate each action's value from a single sampled continuation. The resulting local credit remains sensitive to decisions made later in the trajectory. To address this problem, we propose ConCal (Continuation Calibration), a recursive continuation-value estimator that incorporates continuation evidence already present in a rollout batch. ConCal matches visits from the same task by their incoming state-action-state transitions, combines shared continuation evidence with each visit's own transition estimate, and propagates calibrated values backward to refine earlier action-value estimates. This reduces dependence on individual sampled continuations and mitigates local credit distortions without additional rollouts. Within matched groups, ConCal reduces relative-value error and improves agreement with held-out action orderings compared with estimates from individual continuations. With Qwen2.5-1.5B-Instruct and Qwen2.5-7B-Instruct, ConCal improves mean success rates over GiGPO by 2.87 to 6.78 percentage points on ALFWorld and WebShop. Our code is available at https://github.com/Yingjian-Chen/ConCal.

==> sections/abstract.tex <==
\begin{abstract}
Reinforcement learning for long-horizon agents relies on feedback from sequences of interactions, making credit assignment to individual actions difficult. Existing methods such as GiGPO compare actions at shared states to compute relative advantages, but estimate each action's value from a single sampled continuation. The resulting local credit remains sensitive to decisions made later in the trajectory.
%
To address this problem, we propose \textbf{ConCal} (\textbf{Con}tinuation \textbf{Cal}ibration), a recursive continuation-value estimator that incorporates continuation evidence already present in a rollout batch. ConCal matches visits from the same task by their incoming state-action-state transitions, combines shared continuation evidence with each visit's own transition estimate, and propagates calibrated values backward to refine earlier action-value estimates. This reduces dependence on individual sampled continuations and mitigates local credit distortions without additional rollouts.
%
Within matched groups, ConCal reduces relative-value error and improves agreement with held-out action orderings compared with estimates from individual continuations. With Qwen2.5-1.5B-Instruct and Qwen2.5-7B-Instruct, ConCal improves mean success rates over GiGPO by 2.87–6.78 percentage points on ALFWorld and WebShop. Our code is available at \url{https://github.com/Yingjian-Chen/ConCal}.
\end{abstract}


==> sections/conclusion.tex <==
\section{Conclusion}
We introduce ConCal, a recursive continuation-value estimator for long-horizon agentic reinforcement learning. ConCal combines evidence from matched visits with the transition estimate of each visit and propagates calibrated continuation values to earlier decisions without additional rollouts. Experiments on ALFWorld and WebShop show improved task performance, with ablations supporting both recursive evidence reuse and visit-specific estimation. Further analyses show that shared continuations calibrate preference strength and improve agreement with action orderings derived from held-out returns. These findings support calibrating relative action-value estimates with shared continuation evidence from existing rollout groups in the evaluated settings.





==> sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\paragraph{Benchmarks.}
Following prior work~\citep{feng2025gigpo,cheng2026graphgpo}, our main experiments use ALFWorld~\citep{shridhar2021alfworld} and WebShop~\citep{yao2022webshop}. ALFWorld comprises six categories of household tasks performed through text-based interactions. WebShop requires agents to search for and purchase products that satisfy user requirements. We additionally evaluate ConCal on $6\times6$ Sokoban~\citep{schrader2018gymsokoban,cheng2026graphgpo}, where agents use visual observations to push boxes onto target locations. We report overall and per-category success rates on ALFWorld, average task score and success rate on WebShop, and success rate on Sokoban.

\paragraph{Baselines.}
We compare against GPT-4o~\citep{openai2024gpt4o} and Gemini-2.5-Pro~\citep{comanici2025gemini}, prompting methods ReAct~\citep{yao2023react} and Reflexion~\citep{shinn2023reflexion}, and RL methods PPO~\citep{schulman2017ppo}, RLOO~\citep{ahmadian-etal-2024-back}, GRPO~\citep{shao2024deepseekmath}, GiGPO~\citep{feng2025gigpo}, and GraphGPO~\citep{cheng2026graphgpo}. We also include Qwen2.5-Instruct without additional RL training. 

\paragraph{Implementation Details.} 
On ALFWorld and WebShop, we train Qwen2.5-1.5B-Instruct and Qwen2.5-7B-Instruct for 150 updates, collecting eight trajectories for each of 16 tasks per update. On Sokoban, we train Qwen2.5-VL-3B-Instruct~\citep{bai2025qwen25vl} for 150 updates with 256 trajectories per update and use the native environment rewards. For our training runs, we report means and sample standard deviations across three independent runs. Full training and evaluation settings are provided in Appendix~\ref{app:implementation}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/learning_analysis.pdf}
    \caption{Learning curves of ConCal (green), GiGPO (blue), and GRPO (gray) on ALFWorld and WebShop with Qwen2.5-1.5B-Instruct. Training episode success rates are plotted against policy updates, with faint lines showing unsmoothed curves and bold lines showing EMA-smoothed curves with decay $0.95$.}
    \label{fig:training_dynamics}
\end{figure}

\subsection{Experimental Results}
\paragraph{Main results.} 
\tablename~\ref{tab:main_results} compares ConCal with existing methods on ALFWorld and WebShop. ConCal achieves the highest reported mean success rates on ALFWorld and WebShop at both model sizes. With the 1.5B model, ConCal reaches 95.31\% success on ALFWorld and 79.69\% success on WebShop, with a WebShop task score of 90.59. These success rates exceed GRPO by 17.45 and 8.34 percentage points (pp), respectively, while the WebShop task score is 5.86 points higher. Relative to its base method, GiGPO, ConCal improves success rates by 4.43 pp on ALFWorld and 5.86 pp on WebShop, and increases the WebShop task score by 2.65 points. It also outperforms GraphGPO in overall success rate by 2.60 pp on ALFWorld and 1.04 pp on WebShop. With the 7B model, ConCal reaches 97.14\% success on ALFWorld and 85.16\% success on WebShop, with a WebShop task score of 92.92. On ALFWorld, its success rate is 2.87 pp higher than GiGPO and 1.83 pp higher than GraphGPO. On WebShop, ConCal improves success rates over GiGPO and GraphGPO by 6.78 and 4.85 pp, respectively, and raises task scores by 6.20 and 5.98 points. These results demonstrate the effectiveness of ConCal.

\begin{table}[t]
\centering
\small
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{11pt}
\begin{tabular}{@{}llc@{}}
\toprule
\textbf{Type} & \textbf{Method} & \textbf{Success rate (\%)} \\
\midrule
Prompting   & Qwen2.5-VL     & 11.7 \\
RL Training & GRPO           & 67.1 \\
RL Training & GiGPO          & $76.30_{\pm 1.97}$ \\
RL Training & GraphGPO       & $83.59_{\pm 3.13}$ \\
\rowcolor{gray!15}
RL Training & \textsc{ConCal} & $\mathbf{84.90}_{\pm 2.26}$ \\
\bottomrule
\end{tabular}
\caption{Success rates (\%) on $6\times6$ Sokoban with Qwen2.5-VL-3B-Instruct. We report validation means $\pm$ sample standard deviations for GiGPO, GraphGPO, and ConCal. The prompting and GRPO results are from \citep{cheng2026graphgpo}.}
\label{tab:sokoban_results}
\end{table}

\paragraph{Learning dynamics.}
\figurename~\ref{fig:training_dynamics} compares the training success rates of ConCal, GiGPO, and GRPO on ALFWorld and WebShop. On ALFWorld, ConCal improves more rapidly during the early to middle stages and maintains higher success rates than GiGPO through most of training. On WebShop, ConCal and GiGPO initially follow similar trends, but ConCal achieves higher success rates in later stages and maintains this advantage through the final updates.

\paragraph{Additional evaluation on Sokoban.}
We extend our evaluation from the text-based environments above to $6\times6$ Sokoban, where agents act on visual observations. As shown in \tablename~\ref{tab:sokoban_results}, using Qwen2.5-VL-3B-Instruct, ConCal achieves a mean validation success rate of 84.90\%, exceeding GiGPO by 8.6 pp and GraphGPO by 1.3 pp in our experiments.

Section~\ref{sec:relative_calibration} assesses action-value estimation quality. Sections~\ref{sec:estimator_ablation} and~\ref{sec:normalization} examine estimation components and advantage normalization, Section~\ref{sec:reuse_efficiency} reports reuse coverage and computational cost, and Section~\ref{sec:case_study} presents a case study.

\subsection{Quality of Local Action-Value Estimates}
\label{sec:relative_calibration}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{img/ablation1.pdf}
    \caption{Calibration of relative action values. Agreement and Disagreement indicate whether the estimated action ordering matches or reverses the ordering given by held-out returns. Tie denotes near-equal estimated values. Ordering comparisons exclude action pairs with tied held-out returns. Gap-matched rescales the centered Own-MC values within each group to match the norm of the ConCal estimates while preserving their ordering. MSE measures group-centered value error against held-out returns.}
    \label{fig:relative_calibration}
\end{figure}

To investigate how shared evidence calibrates relative action values, we compare Own-MC and ConCal on the same frozen rollouts on ALFWorld and WebShop, with held-out continuation returns as the reference, following the split described in Appendix~\ref{app:diagnostics}. Own-MC estimates each action value from the Monte Carlo return along the same trajectory, as in GiGPO. We measure group-centered value MSE and action-order agreement to assess the accuracy of value differences and preference direction. Gap-matched serves as a diagnostic control that rescales the centered Own-MC values in each group to the norm of the ConCal estimates while preserving their ordering. This tests how much of the estimation-error reduction can be reproduced by adjusting preference strength alone. \figurename~\ref{fig:relative_calibration} shows that ConCal reduces centered-value MSE by 34.3\% on ALFWorld and 16.8\% on WebShop. Gap-matched reproduces most of the MSE reduction while preserving the Own-MC ordering, showing that much of the error reduction can be recovered by adjusting preference strength alone. ConCal also increases ordering agreement from 58.8\% to 61.2\% and from 74.5\% to 81.8\%, respectively. Within the evaluated comparison groups, these results show that shared continuations improve relative action-value estimates by calibrating preference strength and increasing agreement with the reference ordering.

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{9pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\multirow{2}{*}{Estimator} & ALFWorld & \multicolumn{2}{c}{WebShop} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-4}
& All (\%) & Score & Succ. (\%) \\
\midrule
Own-MC & $90.89 \pm 1.63$ & $88.25 \pm 0.80$ & $73.44 \pm 2.07$ \\
Fully pooled & $91.93 \pm 2.39$ & $89.79 \pm 1.54$ & $\underline{78.65 \pm 4.51}$ \\
Single-pass & $\underline{93.49 \pm 1.97}$ & $\underline{90.25 \pm 2.28}$ & $\underline{78.65 \pm 3.16}$ \\
\textbf{ConCal} & $\mathbf{95.31 \pm 1.35}$ & $\mathbf{90.59 \pm 0.83}$ & $\mathbf{79.69 \pm 3.41}$ \\
\bottomrule
\end{tabular}%
}
\caption{Continuation-estimator ablations on ALFWorld and WebShop. We report overall success rate on ALFWorld and task score and success rate on WebShop, as means $\pm$ sample standard deviations across three runs. The best and second-best means are shown in bold and underlined, respectively.}
\label{tab:estimator_ablation}
\end{table}

\subsection{Component Analysis}
We evaluate continuation estimation through task-performance ablations and normalization through frozen-estimate diagnostics.

\subsubsection{\textbf{Continuation Estimation}}
\label{sec:estimator_ablation}
We further compare ConCal with Own-MC and two variants to examine how continuation estimation contributes to task performance. Single-pass shares continuation returns once, without recursively propagating updated estimates backward. Fully pooled retains recursion but assigns each matched visit the pooled mean, removing its separate visit-specific contribution. All other components and settings remain unchanged. 
\tablename~\ref{tab:estimator_ablation} supports three findings. (1) All three estimators that share continuation evidence (Single-pass, Fully pooled, and ConCal) outperform Own-MC across the reported metrics, supporting the benefit of using evidence from other trajectories. (2) ConCal improves mean success rates over Single-pass by 1.82 percentage points on ALFWorld and 1.04 on WebShop. These gains support propagating calibrated continuation estimates back to earlier decisions. (3) ConCal outperforms Fully pooled across all metrics, indicating that retaining each visit's own estimate remains useful even when continuations are shared. Together, these findings support ConCal's design of recursive evidence reuse with visit-specific estimation.


\subsubsection{\textbf{Advantage Normalization Diagnostic}}
\label{sec:normalization}
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/ablation2.pdf}
    \caption{Relationship between calibrated value spread and step-advantage magnitude under group-wise and batch-wise normalization on ALFWorld and WebShop. Within each batch, state groups with nonzero value spread are divided into five approximately equal-sized bins by the root mean square (RMS) of their centered action values, from bin 1 with the smallest spread to bin 5 with the largest. The vertical axis shows the step-advantage RMS of each group divided by the corresponding batch-level step-advantage RMS. Boxes show the middle 50\% of values, whiskers the 5th--95th percentiles, and lines connect medians.}
    \label{fig:normalization}
    \vspace{-2mm}
\end{figure}

To examine whether normalization preserves the preference strength calibrated by ConCal, we test whether groups with larger value gaps receive stronger step advantages. For this diagnostic comparison, we apply group-wise and batch-wise normalization to the same frozen ConCal estimates and compare step-advantage magnitudes across five bins ordered from smaller to larger value gaps. \figurename~\ref{fig:normalization} shows that group-wise normalization produces similar median advantage magnitudes across bins on both benchmarks. Groups with small calibrated value gaps therefore receive step signals comparable in magnitude to those with large gaps, weakening the distinction between weak and strong estimated action preferences. Under batch-wise normalization, median advantage magnitudes increase with value spread, so smaller gaps receive weaker step signals and larger gaps receive stronger signals. This preserves the preference-strength differences calibrated by ConCal and supports our adoption of batch-wise normalization when computing step advantages.

\subsection{Continuation Reuse and Computational Cost}
\label{sec:reuse_efficiency}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{img/ablation3.pdf}
    \caption{Computational cost and coverage of ConCal. (a) Runtime averaged equally over ALFWorld and WebShop. Blue bars denote common training stages, and green bars denote our visit matching and recursive calibration. The x-axis is broken. (b) Direct coverage denotes actions whose next visits have matches in other trajectories. Indirect coverage denotes additional actions reached through recursive propagation of calibrated continuation values. Gray segments indicate uncovered actions, and brackets show total coverage.}
    \label{fig:reuse_efficiency}
\end{figure}

To assess the computational cost and coverage of ConCal, we examine stage runtimes and the fraction of actions covered by shared continuation evidence. \figurename~\ref{fig:reuse_efficiency}(a) shows that rollout is the most time-consuming training stage, taking 108.85\,s on average, followed by policy updates at 19.00\,s. In separate frozen-batch replays, visit matching and recursive calibration for ConCal take 0.0375\,s and 0.0019\,s per batch, respectively, under the measurement setup in Appendix~\ref{app:diagnostics}. \figurename~\ref{fig:reuse_efficiency}(b) shows that directly matched next visits provide shared continuation evidence for 55.4\% of recorded actions on ALFWorld and 43.4\% on WebShop. Recursive propagation extends this coverage to 92.5\% and 67.5\%, respectively, allowing earlier actions to access shared continuation evidence even when their immediate successor visits have no cross-trajectory matches. ConCal therefore makes shared continuation evidence available to a broad fraction of recorded actions at a small measured cost for matching and calibration, without collecting additional rollouts.

\subsection{Case study}
\label{sec:case_study}
We present a WebShop case study of local credit assignment for web agents (\figurename~\ref{fig:webshop_case}). The task requires Zest color and size 5X, but the agent has selected only the color. GiGPO estimates each action's value from its own sampled continuation. It assigns negative step advantage to \textit{Select 5X} because its continuation ends in task failure, while favoring \textit{Repeat Zest}, whose trajectory succeeds, yielding a value gap of $\Delta G=-6.9834$. ConCal calibrates action-value estimates using evidence from multiple continuations and reverses this preference, with $\Delta\widetilde Q=+0.6452$. It assigns positive step advantage to \textit{Select 5X} despite its failed sampled continuation, favoring completion of the required size selection. This case illustrates how ConCal uses shared continuation evidence to assign positive local credit to useful actions despite failures in their own sampled continuations.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{img/case_study.pdf}
    \caption{Case study in WebShop. Both panels evaluate the same two trajectories. Both gaps subtract the estimate for repeating Zest from that for selecting 5X. Green dashed links indicate shared continuation evidence; two of the three matched visits are shown. Webpages are reconstructed from recorded states using the official interface.}
    \label{fig:webshop_case}
\end{figure}



==> sections/introduction.tex <==
\section{Introduction}
\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{img/overview.pdf}
    \caption{Comparison of credit assignment strategies.
    (a) GRPO assigns the same trajectory-level credit to all actions.
    (b) GiGPO compares actions at shared state anchors based on their own sampled returns.
    (c) Our proposed ConCal estimates local action values from continuation evidence shared among matched visits across rollouts. Visits from the same task are matched by their preceding state, executed action, and current state.}
    \label{fig:motivation}
\end{figure}

Large language models (LLMs)~\citep{openai2023gpt4,qwen2.5} support agents that reason, invoke tools, and interact with external environments~\citep{yao2023react,schick2023toolformer}. In web navigation and embodied tasks~\citep{he-etal-2024-webvoyager,ichter2023saycan}, agents execute sequences of actions and adapt their decisions to changing observations~\citep{xi-etal-2025-agentgym}. Reinforcement learning (RL) trains these behaviors from task outcomes~\citep{wei-etal-2025-webagent,wang2025ragen,jin2025searchr1}. A central challenge is to translate feedback on the full interaction into credit for individual decisions.

Group-based RL estimates relative advantages from trajectories sampled for the same task. In trajectory-level GRPO~\citep{shao2024deepseekmath}, every action in a trajectory receives the same episode-relative advantage, as illustrated in \figurename~\ref{fig:motivation}(a). GiGPO~\citep{feng2025gigpo} introduces local comparisons by grouping actions at shared state anchors and comparing their discounted returns, as illustrated in \figurename~\ref{fig:motivation}(b). The comparison is local, but the value estimate for each action still comes from its own sampled continuation. Consequently, a low return does not distinguish a poor decision from a useful decision followed by later failure. Similarly, a high return does not identify which earlier decisions contributed to success. The credit conflicts in \figurename~\ref{fig:analysis} illustrate the variability of these estimates on subsets of WebShop~\citep{yao2022webshop} and ALFWorld~\citep{shridhar2021alfworld} rollouts. State grouping determines which actions are compared, while continuation estimation determines the values entering that comparison.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{img/aaa.pdf}
    \caption{Credit-conflict rates and centered-value MSE on WebShop and ALFWorld. \textit{Credit conflict (\%)} measures the proportion of repeated-decision groups in which the same recorded decision receives both positive and negative local credit. \textit{Centered-value MSE} measures group-centered estimation error against held-out returns. For illustration, both estimators are evaluated on the same subset of 1,000 existing rollout trajectories from each benchmark.}
    \label{fig:analysis}
\end{figure}

The rollout batch also contains evidence beyond each individual continuation. Existing approaches reuse cross-trajectory structure through transition-level advantage averaging and graph-based credit estimation~\citep{li-etal-2026-salt,cheng2026graphgpo,yao2026graft}. For a given task, repeated transitions with the same starting state, executed action, and resulting state link that action to several observed continuations, as illustrated in \figurename~\ref{fig:motivation}(c). The visits following these transitions provide shared evidence about subsequent returns, while each visit records a particular reward and successor within its own trajectory. A single pooled value removes these differences from the estimates assigned to matched visits. Our insight is to calibrate action values by combining shared continuation evidence with each visit's own transition estimate and propagating the resulting estimates backward to earlier decisions.

Accordingly, we propose \textbf{Con}tinuation \textbf{Cal}ibration (\textbf{ConCal}), a recursive estimator of continuation values. ConCal matches visits by their incoming state-action-state transitions and blends the transition estimate of each visit with the mean estimate of matched visits. This partial sharing retains a separate estimate for each visit. Recursive updates carry the calibrated continuation values backward along recorded trajectories, allowing earlier action-value estimates to incorporate evidence from other rollouts. Each action is evaluated from its own observed reward and the calibrated continuation value of its actual successor, without collecting additional rollouts. The illustrative held-out diagnostics in \figurename~\ref{fig:analysis} show lower error in relative values and greater local credit consistency than estimates based on individual continuations.

In summary, our contributions are as follows: 
\textbf{(1) Analysis of Local Credit Assignment.}
We analyze the dependence of return-based local credit on individual sampled continuations through credit-conflict measurements and held-out relative-value diagnostics.
\textbf{(2) Calibrating Local Action Values.}
We introduce ConCal, which combines shared continuation evidence from matched visits with each visit's own transition estimate through recursive updates to refine local action-value estimates within the existing rollout batch.
\textbf{(3) Empirical Evaluation.}
With Qwen2.5-1.5B-Instruct, ConCal improves success rates over GiGPO by 4.43 and 5.86 percentage points on ALFWorld and WebShop, respectively, and achieves higher reported mean success rates than GraphGPO on both benchmarks. Ablations support recursive sharing and retention of individual transition estimates, while diagnostics examine relative-value magnitudes and action orderings.



==> sections/limitations.tex <==
\section*{Limitations}
The matching rule of ConCal relies on observed incoming transitions and does not enforce agreement in the full interaction history, hidden state, or remaining interaction budget. Such differences can introduce bias into the shared estimates incorporated into subsequent recursive updates. The extent of continuation reuse also depends on the availability of matching visits within the rollout batch. Future work could refine matching with relevant historical information while maintaining sharing coverage, and account for uncertainty in continuation estimates.



==> sections/method.tex <==
\section{Continuation Calibration}
We introduce \textsc{ConCal}, a recursive continuation-value estimator that evaluates actions from continuation evidence shared across existing rollouts. \figurename~\ref{fig:method} illustrates three steps. \textbf{Matching Visits} identifies visits that share continuation evidence. \textbf{Recursive Continuation Calibration} blends individual transition estimates with the matched mean. \textbf{Action Values and Policy Optimization} converts calibrated continuation values into action values and relative advantages for policy updates.

\subsection{Matching Visits}
To construct the estimator $\mathcal E(\mathcal D,i,t)$ introduced in Section~\ref{sec:problem_formulation}, we first match visits across trajectories by the task, preceding state, executed action, and current state. Matching the incoming transition distinguishes visits that reach the same observed state through different preceding state-action pairs. For visit $(i,t)$, the matching key is
\begin{equation}
    z_t^{(i)}
    =
    \left(
        x,\,
        s_{t-1}^{(i)},\,
        a_{t-1}^{(i)},\,
        s_t^{(i)}
    \right).
    \label{eq:context_key}
\end{equation}
At $t=0$, a start marker replaces the preceding state and action. We collect visits with the same $z$ into a sharing pool:
\begin{equation}
    \mathcal C(z)=\{(j,k)\mid z_k^{(j)}=z\},
    \label{eq:context_pool}
\end{equation}
where $(j,k)$ denotes the visit at step $k$ of trajectory $\tau_j$ in $\mathcal D$. Matched visits need not occur at the same time step.

To evaluate action $a_t^{(i)}$, we draw on the pool $\mathcal C(z_{t+1}^{(i)})$ to calibrate the continuation value at its actual successor visit $(i,t+1)$ when $t+1<T_i$. For example, in \figurename~\ref{fig:method}, the tuples $(s_2^{(i)},a_2^{(i)},s_3^{(i)})$ match for $i\in\{1,2,3\}$, so the continuations from these visits at $s_3^{(i)}$ provide shared evidence for evaluating $a_2^{(2)}$.

\subsection{Recursive Continuation Calibration}
The continuation value at a visit depends on its immediate reward and the value of its actual successor. ConCal calibrates this value with evidence from matched visits while retaining a separate estimate for each visit. Let $\widehat V_b(s_t^{(i)})$ denote the continuation estimate for visit $(i,t)$ at recursion depth $b$, initialized as $\widehat V_0(s_t^{(i)})=0$.

\paragraph{Visit-specific calibration.}
We first compute the transition estimate for each visit:
\begin{equation}
    Y_{t,b}^{(i)}
    =
    r_t^{(i)}
    +
    \gamma\widehat V_{b-1}(s_{t+1}^{(i)}).
    \label{eq:own_transition_estimate}
\end{equation}
The successor term is zero when no successor visit is recorded, including at collection truncations.

The pool mean averages the transition estimates of all matched visits, including the current visit:
\begin{equation}
    \mu_b(z)
    =
    \frac{1}{|\mathcal C(z)|}
    \sum_{(j,k)\in\mathcal C(z)}
    Y_{k,b}^{(j)}.
    \label{eq:context_mean}
\end{equation}
ConCal then calibrates the continuation value at each visit by blending its transition estimate with the pool mean:
\begin{equation}
    \widehat V_b(s_t^{(i)})
    =
    (1-\alpha_z)Y_{t,b}^{(i)}
    +
    \alpha_z\mu_b(z),
    \label{eq:continuation_calibration}
\end{equation}
where $z=z_t^{(i)}$, $\alpha_z=\frac{n_z}{n_z+1}$, and $n_z$ is the number of distinct trajectories in $\mathcal C(z)$. This calibration moves the estimate for each visit toward the shared mean while retaining its own transition contribution. The pool mean averages visits, and its weight increases with the number of distinct contributing trajectories.

At a fixed sharing pool and recursion depth, calibration preserves the mean of the transition estimates and contracts their pairwise differences. For any $(i,t),(j,k)\in\mathcal C(z)$,
\begin{equation}
    \widehat V_b(s_t^{(i)})
    -
    \widehat V_b(s_k^{(j)})
    =
    \frac{
    Y_{t,b}^{(i)}-Y_{k,b}^{(j)}
    }{n_z+1}.
    \label{eq:visit_difference}
\end{equation}
Each visit therefore retains its own deviation from the shared mean, scaled by $1/(n_z+1)$.

\paragraph{Recursive propagation.}
In \figurename~\ref{fig:method}, each recursive update combines the transition estimate for visit $(2,3)$ with the mean of the three matched estimates to calibrate its continuation value. This computation repeats for $b=1,\ldots,H$, where $H$ is the maximum interaction budget. At depth $b$, all visits incorporate successor estimates from depth $b-1$. The calibrated values then enter the transition estimates of preceding visits at the next depth, propagating shared continuation evidence backward through recorded transitions.

\subsection{Action Values and Policy Optimization}
The recursively calibrated continuation values provide the basis for action evaluation. Each action retains its observed reward and actual successor:
\begin{equation}
    \widetilde Q_t^{(i)}
    =
    r_t^{(i)}
    +
    \gamma\widehat V_{H-t-1}(s_{t+1}^{(i)}),
    \label{eq:concal_action_value}
\end{equation}
where $t=0,\ldots,T_i-1$. The successor estimate is taken at recursion depth $H-t-1$, corresponding to the remaining interaction budget after the action. The successor term follows the boundary convention defined above.

Batch-wise normalization converts the calibrated action values into step advantages by centering them within each state group and applying a shared batch-level scale. The resulting step advantages are combined with the episode-level advantage in GiGPO:

\begin{equation}
\begin{aligned}
    \widetilde A_t^{S,(i)}
    &=
    \frac{
    \widetilde Q_t^{(i)}
    -
    \overline{\widetilde Q}_{\mathcal S_t^{(i)}}
    }{\widetilde d_{\mathcal B}},\\
    \widetilde A_t^{(i)}
    &=
    A^{E,(i)}
    +
    \beta\widetilde A_t^{S,(i)},
\end{aligned}
\label{eq:calibrated_local_advantage}
\end{equation}
where $\overline{\widetilde Q}_{\mathcal S}$ is the mean action-value estimate within the group, $\widetilde d_{\mathcal B}$ is a normalization scale shared across the batch, and $\beta$ balances episode-level and step-level credit. On WebShop, the shared scale is one, which reduces step-advantage normalization to mean centering. Details are provided in Appendix~\ref{app:step_normalization}.

\begin{table*}[t]
\centering
\begingroup
\fontsize{12}{13.5}\selectfont
\setlength{\tabcolsep}{2.6pt}
\renewcommand{\arraystretch}{1.3}
\newcommand{\srval}[2]{$#1_{\pm #2}$}
\newcommand{\bsrval}[2]{\begingroup\boldmath$#1_{\pm #2}$\endgroup}
\newcommand{\usrval}[2]{\underline{$#1_{\pm #2}$}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llccccccccc@{}}
\toprule
Type & Method & \multicolumn{7}{c}{ALFWorld}
& \multicolumn{2}{c}{WebShop} \\
\cmidrule(lr){3-9}\cmidrule(l){10-11}
& & Pick & Clean & Cool & Look & Heat & Pick2 & All
& Score & Succ. \\
\midrule
\multicolumn{11}{@{}l}{\textit{Closed-Source Models}} \\
Prompting & GPT-4o
& 75.3 & 60.8 & 31.2 & 56.7 & 21.6 & 49.8 & 48.0
& 31.8 & 23.7 \\
Prompting & Gemini-2.5-Pro
& 92.8 & 63.3 & 62.1 & 69.0 & 26.6 & 58.7 & 60.3
& 42.5 & 35.9 \\
\midrule
\multicolumn{11}{@{}l}{\textit{Qwen2.5-1.5B-Instruct}} \\
Prompting & Qwen2.5
& 5.9 & 5.5 & 3.3 & 9.7 & 4.2 & 0.0 & 4.1
& 23.1 & 5.2 \\
Prompting & ReAct
& 17.4 & 20.5 & 15.7 & 6.2 & 7.7 & 2.0 & 12.8
& 40.1 & 11.3 \\
Prompting & Reflexion
& 35.3 & 22.2 & 21.7 & 13.6 & 19.4 & 3.7 & 21.8
& 55.8 & 21.9 \\
RL Training & PPO (with critic)
& \srval{64.8}{3.5}
& \srval{40.5}{6.9}
& \srval{57.1}{4.9}
& \srval{60.6}{6.6}
& \srval{46.4}{4.0}
& \srval{47.4}{1.9}
& \srval{54.4}{3.1}
& \srval{73.8}{3.0}
& \srval{51.5}{2.9} \\
RL Training & RLOO
& \srval{88.3}{3.0}
& \srval{52.8}{8.6}
& \srval{71.0}{5.9}
& \srval{62.8}{8.7}
& \srval{66.4}{5.5}
& \srval{56.9}{4.7}
& \srval{69.7}{2.5}
& \srval{73.9}{5.6}
& \srval{52.1}{6.7} \\
RL Training & GRPO
& \srval{82.89}{3.62}
& \srval{82.14}{6.37}
& \srval{73.86}{6.84}
& \srval{78.57}{0.00}
& \srval{77.78}{4.54}
& \srval{71.43}{3.89}
& \srval{77.86}{1.33}
& \srval{84.73}{0.49}
& \srval{71.35}{2.05} \\
RL Training & GiGPO$^{*}$
& \bsrval{98.81}{1.68}
& \srval{95.16}{3.89}
& \srval{81.46}{0.56}
& \srval{78.57}{0.00}
& \srval{94.44}{0.00}
& \bsrval{93.65}{5.94}
& \srval{90.88}{0.97}
& \srval{87.94}{0.43}
& \srval{73.83}{2.30} \\
RL Training & GraphGPO
& \srval{95.15}{1.62}
& \bsrval{100.00}{0.00}
& \usrval{85.26}{2.58}
& \usrval{85.71}{5.83}
& \usrval{96.30}{2.61}
& \bsrval{93.65}{2.24}
& \usrval{92.71}{1.32}
& \usrval{89.29}{1.48}
& \usrval{78.65}{3.86} \\
\rowcolor{blue!7}
RL Training & \textsc{ConCal}
& \usrval{97.70}{2.00}
& \usrval{98.48}{2.62}
& \bsrval{90.61}{8.88}
& \bsrval{90.11}{8.58}
& \bsrval{98.15}{3.21}
& \usrval{92.82}{3.11}
& \bsrval{95.31}{1.35}
& \bsrval{90.59}{0.83}
& \bsrval{79.69}{3.41} \\
\midrule
\multicolumn{11}{@{}l}{\textit{Qwen2.5-7B-Instruct}} \\
Prompting & Qwen2.5
& 33.4 & 21.6 & 19.3 & 6.9 & 2.8 & 3.2 & 14.8
& 26.4 & 7.8 \\
Prompting & ReAct
& 48.5 & 35.4 & 34.3 & 13.2 & 18.2 & 17.6 & 31.2
& 46.2 & 19.5 \\
Prompting & Reflexion
& 62.0 & 41.6 & 44.9 & 30.9 & 36.3 & 23.8 & 42.7
& 58.1 & 28.8 \\
RL Training & PPO (with critic)
& \srval{92.3}{4.0}
& \srval{64.0}{8.4}
& \usrval{92.5}{2.4}
& \srval{89.5}{7.0}
& \srval{80.3}{2.0}
& \srval{68.8}{8.3}
& \srval{80.4}{2.7}
& \srval{81.4}{3.1}
& \srval{68.7}{5.1} \\
RL Training & RLOO
& \srval{87.6}{4.3}
& \srval{78.2}{8.3}
& \srval{87.3}{5.8}
& \srval{81.3}{7.6}
& \srval{71.9}{5.2}
& \srval{48.9}{8.4}
& \srval{75.5}{4.6}
& \srval{80.3}{3.2}
& \srval{65.7}{4.0} \\
RL Training & GRPO
& \srval{88.98}{5.30}
& \srval{91.98}{4.43}
& \srval{77.89}{4.58}
& \srval{78.57}{0.00}
& \srval{90.74}{5.24}
& \srval{71.43}{3.89}
& \srval{83.33}{2.05}
& \srval{84.31}{1.27}
& \srval{75.00}{2.78} \\
RL Training & GiGPO$^{*}$
& \usrval{97.53}{1.75}
& \bsrval{100.00}{0.00}
& \srval{83.98}{1.32}
& \usrval{90.48}{6.73}
& \usrval{94.44}{0.00}
& \bsrval{100.00}{0.00}
& \srval{94.27}{1.33}
& \srval{86.72}{1.44}
& \srval{78.38}{1.94} \\
RL Training & GraphGPO
& \bsrval{100.00}{0.00}
& \bsrval{100.00}{0.00}
& \srval{91.40}{1.50}
& \bsrval{92.86}{5.83}
& \usrval{94.44}{0.00}
& \srval{92.06}{2.24}
& \usrval{95.31}{1.10}
& \usrval{86.94}{0.68}
& \usrval{80.31}{1.33} \\
\rowcolor{blue!7}
RL Training & \textsc{ConCal}
& \bsrval{100.00}{0.00}
& \usrval{97.22}{2.41}
& \bsrval{92.80}{6.46}
& \srval{88.89}{19.25}
& \bsrval{100.00}{0.00}
& \usrval{95.11}{4.84}
& \bsrval{97.14}{0.45}
& \bsrval{92.92}{1.36}
& \bsrval{85.16}{2.07} \\
\bottomrule
\end{tabular}}
\endgroup
\caption{Performance on ALFWorld and WebShop with Qwen2.5-1.5B-Instruct and Qwen2.5-7B-Instruct. For ALFWorld, we report per-category and overall success rates (\%). For WebShop, we report average task scores and success rates (\%). ConCal results report validation means $\pm$ sample standard deviations across three runs. $^{*}$ marks the base method on which ConCal builds. Baseline results are taken from prior publications~\citep{feng2025gigpo,cheng2026graphgpo}. The best and second-best means are shown in bold and underlined, respectively.}
\label{tab:main_results}
\end{table*}

We then optimize the following clipped objective with the combined advantages:
\begin{equation}
\begin{aligned}
&\mathcal J(\theta)
=
\mathbb E_{\mathcal B\sim\pi_{\mathrm{old}}}
\Biggl[
\sum_{k=1}^{L} w_k
\min\Bigl(
\rho_k\widetilde A_k,\\
&\operatorname{clip}\bigl(
\rho_k,1-\epsilon,1+\epsilon
\bigr)\widetilde A_k
\Bigr)
-\lambda_{\mathrm{KL}}
\mathbb D_{\mathrm{KL}}
(\pi_\theta\|\pi_{\mathrm{ref}})
\Biggr],
\end{aligned}
\label{eq:concal_policy_objective}
\end{equation}
where $L$ is the number of generated tokens, $w_k$ denotes the normalized actor-loss weight of token $k$ with $\sum_k w_k=1$, and $\widetilde A_k$ is the combined advantage of the step containing that token. The importance ratio is $\rho_k=\pi_\theta(a_k\mid h_k)/\pi_{\mathrm{old}}(a_k\mid h_k)$, where $a_k$ is the generated token and $h_k$ contains the policy input context and preceding tokens within the action. The clipping threshold is $\epsilon$, and $\lambda_{\mathrm{KL}}$ controls the KL penalty relative to the reference policy $\pi_{\mathrm{ref}}$. The KL term denotes the weighted average over token contexts $h_k$ with weights $w_k$. The advantages remain fixed during optimization. Algorithm~\ref{alg:concal} in Appendix~\ref{app:algorithm} summarizes the action-value estimation procedure.




==> sections/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

\subsection{Group-Based Agent RL}
\label{sec:setup_gigpo}
We consider language agents that interact sequentially with an environment to complete tasks. Given a task $x$, the agent receives an observed state $s_t$ and generates a textual action $a_t$ based on the current state and retained interaction history. The environment returns a reward $r_t$ and the next state $s_{t+1}$. Rewards reflect the terminal task outcome, with intermediate task rewards set to zero. At each training iteration, the rollout policy $\pi_0=\pi_{\mathrm{old}}=\pi_{\theta_{\mathrm{old}}}$ is held fixed to collect $N$ trajectories per task. For a given task $x$, let $\mathcal D=\{\tau_i\}_{i=1}^{N}$ denote its rollout group. The full training batch $\mathcal B$ contains the rollout groups for all sampled tasks. Each trajectory $\tau_i$ contains $T_i\leq H$ transitions $(s_t^{(i)},a_t^{(i)},r_t^{(i)},s_{t+1}^{(i)})$, where $H$ is the maximum number of interactions. Each decision step $(i,t)$, with $0\le t<T_i$, constitutes a \emph{visit} to the observed state $s_t^{(i)}$.

\paragraph{Episode-level advantages.}
GRPO compares returns within a rollout group~\citep{shao2024deepseekmath}. For the total task return $R(\tau_i)=\sum_{t=0}^{T_i-1}r_t^{(i)}$, the episode-relative advantage is
\begin{equation}
    A^{E,(i)}
    =
    \frac{R(\tau_i)-\bar R}{d_E},
    \label{eq:episode_advantage}
\end{equation}
where $\bar R$ is the mean trajectory return. Standard GRPO sets $d_E=\sigma_R+\epsilon_{\mathrm{num}}$, with $\sigma_R$ denoting the standard deviation and $\epsilon_{\mathrm{num}}>0$ a numerical stabilizer. Mean centering instead sets $d_E=1$. All actions in a trajectory share the same episode-level advantage.

\paragraph{Step-level advantages.}
GiGPO introduces local comparisons at repeated state anchors~\citep{feng2025gigpo}. Each action is evaluated by its sampled discounted return 
$
    G_t^{(i)}
    =
    \sum_{u=t}^{T_i-1}\gamma^{u-t}r_u^{(i)},
$
where $\gamma\in[0,1]$ is the discount factor. Let $\mathcal S_t^{(i)}$ contain all visits in $\mathcal D$ sharing the state anchor of visit $(i,t)$. The local advantage and combined training signal are
\begin{equation}
\begin{aligned}
    A_t^{S,(i)}
    &=
    \frac{G_t^{(i)}-\bar G_{\mathcal S_t^{(i)}}}
         {d_{\mathcal S_t^{(i)}}},\\
    A_t^{(i)}
    &=
    A^{E,(i)}+\beta A_t^{S,(i)},
\end{aligned}
\label{eq:gigpo_local_advantage}
\end{equation}
where $\bar G_{\mathcal S}$ is the group mean, $d_{\mathcal S}$ is the normalization scale, and $\beta\geq0$ weights the local advantage. The combined advantages drive PPO-style policy optimization~\citep{schulman2017ppo}.

\subsection{Local Action-Value Estimation}
\label{sec:problem_formulation}

Let $h_t$ denote the full observed interaction history before action $a_t$, including the task, current state, and remaining interaction budget. The action value under $\pi_0$ is
\begin{equation}
    Q^{\pi_0}(h,a)
    =
    \mathbb E_{\pi_0}
    \left[G_t\mid h_t=h,\ a_t=a\right],
    \label{eq:local_action_value}
\end{equation}
where $G_t$ is the discounted return over the remaining episode. The expectation accounts for subsequent policy decisions and environment transitions.

GiGPO relies on one sampled return $G_t^{(i)}$ to estimate $Q^{\pi_0}(h_t^{(i)},a_t^{(i)})$. Although state grouping supplies a local comparison baseline, each estimate still depends on a single sampled continuation. We seek an estimator $\widetilde Q_t^{(i)}=\mathcal E(\mathcal D,i,t)$ that incorporates continuation evidence from matched visits across trajectories to improve local action-value estimates without additional rollouts.




==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\paragraph{Reinforcement learning for language agents.}
Reinforcement learning (RL) has been applied to align language models with human preferences~\citep{ouyang2022training} and train agents through interaction with external environments~\citep{carta2023grounding}. Multi-turn RL enables agents to learn sequential decision-making from environment feedback~\citep{zhou2024archer}, with applications spanning device control~\citep{bai2024digirl}, web navigation~\citep{wei-etal-2025-webagent}, and search-augmented reasoning~\citep{jin2025searchr1}. Recent frameworks further support long-horizon training across diverse interactive environments~\citep{xi2026agentgymrl}. Our work focuses on credit assignment in long-horizon agentic RL.

\paragraph{Group-based local credit assignment.}
Group-based RL estimates relative advantages from sampled rewards without a learned value baseline~\citep{ahmadian-etal-2024-back,shao2024deepseekmath}. Subsequent work improves optimization and sampling to address training bias and instability~\citep{liu2025understanding,yu2025dapo}. For multi-turn agents, local comparisons extend from shared state anchors to groups that account for historical context~\citep{feng2025gigpo,he2026hgpo}. Our work focuses on calibrating the action-value estimates entering these local comparisons through shared continuation evidence from matched visits.

\paragraph{Cross-trajectory credit estimation.}
Shared structure across trajectories provides additional evidence for step-level credit assignment. Tree-GRPO adopts tree-search sampling and computes relative advantages within and across trees~\citep{ji2026tree}. SALT averages trajectory-level advantages over matched state-action-state transitions~\citep{li-etal-2026-salt}. GraphGPO aggregates rollouts into a state-transition graph and derives step-level credit from shortest-path distances to successful terminal states~\citep{cheng2026graphgpo}. GRAFT estimates state values through Bellman updates on a trajectory graph and derives step-level credit from these values~\citep{yao2026graft}. PGPO augments step-level advantages by incorporating differences between state potentials estimated from grouped returns~\citep{zheng2026pgpo}. In this paper, we introduce ConCal to calibrate local action values by recursively combining shared continuation evidence with visit-specific transition estimates, with an in-depth analysis revealing how calibration and normalization shape action preferences and local credit.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\textwidth]{./img/pipeline.pdf}
    \caption{\textbf{Overview of ConCal.} (1) ConCal matches visits across same-task rollouts by their preceding state, executed action, and current state to identify shared continuation evidence (\textbf{Left}). (2) It recursively combines continuation evidence from matched visits while retaining each visit's own transition contribution, producing calibrated continuation values for action evaluation. At each recursion depth, all visits are updated using successor estimates from the previous depth (\textbf{Right}). (3) Each action is evaluated using its immediate reward and its actual successor's calibrated continuation value. The resulting action values are compared within state groups to obtain local advantages, which are combined with episode-level advantages for PPO updates (\textbf{Bottom}).}
    \label{fig:method}
\end{figure*}
